Complementary Information Mutual Learning for Multimodality Medical Image Segmentation

Radiologists must utilize multiple modal images for tumor segmentation and diagnosis due to the limitations of medical imaging and the diversity of tumor signals. This leads to the development of multimodal learning in segmentation. However, the redundancy among modalities creates challenges for existing subtraction-based joint learning methods, such as misjudging the importance of modalities, ignoring specific modal information, and increasing cognitive load. These thorny issues ultimately decrease segmentation accuracy and increase the risk of overfitting. This paper presents the complementary information mutual learning (CIML) framework, which can mathematically model and address the negative impact of inter-modal redundant information. CIML adopts the idea of addition and removes inter-modal redundant information through inductive bias-driven task decomposition and message passing-based redundancy filtering. CIML first decomposes the multimodal segmentation task into multiple subtasks based on expert prior knowledge, minimizing the information dependence between modalities. Furthermore, CIML introduces a scheme in which each modality can extract information from other modalities additively through message passing. To achieve non-redundancy of extracted information, the redundant filtering is transformed into complementary information learning inspired by the variational information bottleneck. The complementary information learning procedure can be efficiently solved by variational inference and cross-modal spatial attention. Numerical results from the verification task and standard benchmarks indicate that CIML efficiently removes redundant information between modalities, outperforming SOTA methods regarding validation accuracy and segmentation effect.

==> experiments.tex <==
This section provides an evaluation of the proposed TEPO on the \texttt{BraTS2020} benchmark, which is a prevalent dataset used for MIS tasks. We aim to address the following key questions, and the following evaluation will focus on answering these questions comprehensively, i.e.,

\smallskip
\noindent {{a) Does the SAM with multi-step interaction outperform the SAM with single-step interaction?}

\noindent b) Can the policies learned by the TEPO algorithm outperform the rule-based policies?

\noindent c) What strategies can be learned from TEPO?

\noindent d) How stable are the strategies learned by TEPO?

\subsection{Dataset and Training Details}

SAM requires 2D images as input and 3D images are conventionally often annotated by viewing them in slices, we adopt the practice of slicing the 3D magnetic resonance scans into axial slices, a method commonly used in related research efforts~\citep{wolleb2022diffusion}.

To evaluate the effectiveness of TEPO in the context of multi-step interaction, we carefully selected slices with sufficiently large foregrounds in the image. 
Specifically, we segment the \textit{Whole Tumor} (WT) from the \textit{FLAIR} images and choose slices that contain a minimum of 256 foreground pixel points for analysis. This carefully curated dataset enables accurate evaluation of the performance and potential of TEPO in future applications in MIS.

The dataset for evaluation comprised a total of 369 patients. 
We split the dataset into three subsets: the training set evaluated $319$ patients and included $17,396$ slices; the validation set consisted of $20$ patients, corresponding to $1,450$ slices; and the test set included $20$ patients with $1,389$ slices.

We crop the images to $200 \times 150$, implement \textit{random flip}, \textit{rotate}, \textit{add noise}, \textit{affine transform} data augmentation to the training dataset, and then rescale the intensity values.
We train for $100$ epochs, and in each epoch, $10,000$ steps are sampled, and the $Q$ network of TEPO is updated $100$ times.
The model is trained with a learning rate of $1e^{-3}$ for the \texttt{Adam} optimizer and a batch size of $64$.


\subsection{Main Results}\label{sec:results}

\input{tabs/tepo_tab}
 
The performance of the proposed TEPO algorithm is evaluated on the \texttt{BraTS2020} dataset for medical image segmentation tasks and compared with three rule-based policy baselines: the one-step oracle agent, the random agent, and the alternately changing agent.
The one-step oracle agent is an optimal decision-making agent that has access to comprehensive information and can observe the reward after adapting various interaction forms.
This allows it to achieve the highest accuracy in a single step and to explore efficient interaction strategies for the given task.
The random agent, on the other hand, uniformly samples actions from available action sets and can be used to simulate clinicians without any preference for any particular interaction form for the task at hand.
The alternately changing agent applies a policy that alternately chooses the forehead point and the background point.

We conduct training on several different reinforcement learning policies with varying horizon settings ($N=\{2,3,5,7,9\}$) and evaluate the agents' performance through the dice score, computed using a ground truth mask and measurements.
At each timestep, the agent first chooses an action to indicate what form of interaction is required. 
To simulate a clinician's behavior, we use rules consisting of choosing specific positions, such as the forehead, background, and center, and drawing bounding boxes around the forehead region.
Specifically, we select the forehead, background, and center points that are farthest from the boundaries of the false negative, false positive, and error regions, respectively. 
For the bounding box, we extend the forehead region by $10$ pixels and draw a rectangle.

\begin{figure}[htb!]
  \centering
  \subfigure[Complete view.]{
    \label{fig:subfig1}
    \includegraphics[width=0.45\textwidth]{imgs/dice.png}}
  \subfigure[Enlarged view.]{
    \label{fig:subfig2}
    \includegraphics[width=0.45\textwidth]{imgs/dice_large.png}}
  \caption{The performance improvement of different IMIS methods at different interaction steps. All these test results are performed on the \texttt{BraTS2020} dataset. Subfigure (a) illustrate various IMIS methods from step one to step nine. To compare the performances of the algorithms, Subfigure (b) shows an enlarged view of steps four to nine, only including those with dice scores larger than 0.75.}
    \label{fig:dice}
\end{figure}


\begin{figure*}[htb!]
    \centering
    \includegraphics[width=0.9\linewidth]{imgs/case_study.png}
    \caption{Visualization of strategies and results of different strategies on the same medical image. The green pentagram indicates the foreground, the red pentagram indicates the background, and the green box indicates the bounding box.}
    \label{fig:case_study}
\end{figure*}

The comparison of the performance of various interaction strategies is evaluated with respect to the number of interactions.
As shown in Figure \ref{fig:dice}, the different lines correspond to the different agents' performance.
``TEPO-X'' indicates that the agent is trained in the $X$-step interaction scenario. 
For example, ``TEPO-$2$'' means a two-step scenario. 
``Random'' denotes the random agent, ``Alternately'' denotes the alternately changing agent, and ``$1$-step Oracal'' denotes the one-step Oracal agent.
We will use the same labeling convention throughout the paper unless noted otherwise.
It is worth noting that we train in different interaction step scenarios, but in testing, we use $9$-step interactions to find out comprehensive performances.

\subsubsection{Quantitative experimental analysis}

\paragraph{Q\#a: Does the SAM in multi-step interaction mode outperform the SAM in single-step interaction mode?} 
As illustrated in Figure \ref{fig:dice}, the TEPO-$2$ agent stays the same after the third round, this is because in our experiments, if the shortest distance of all points from the edge in the corresponding region is less than two pixels, then the user does not interact anymore.
Table \ref{tab:tepo_tab} indicates that the TEPO-$2$ policy predominantly selects the forehead point starting from step two. 
However, the false negative region is too small to click, so the TEPO-$2$ policy stops interacting at step five for all test cases.
Conversely, the performance of other multi-step policies improves with an increase in the number of interactions, showcasing that SAM can be enhanced through multiple rounds of interactions.
Moreover, expect TEPO-$2$, other policies perform better than the one-step Oracle agent, implying that multi-step interactions are more effective for medical image segmentation than the single-step interaction mode.

\paragraph{Q\#b: Can the policies learned by the TEPO algorithm outperform the rule-based policies?}
The experimental results in Figure \ref{fig:dice} indicate that the TEPO-$2$ policy performs better than random and alternating selection methods during the initial two interactions. Moreover, the performance of all other RL-based policies is superior to rule-based approaches. 
These findings provide evidence that the TEPO algorithm significantly boosts the efficacy of SAM in interactive medical scenarios, even in zero-shot mode.

\paragraph{Q\#c: What strategies can be learned from the TEPO algorithm?}
As the TEPO algorithm is trained under different interaction round scenarios, the learned strategies exhibit variations, as summarized in Table \ref{tab:tepo_tab}.
TEPO-$2$ employs a straightforward strategy: selecting the bounding box in the first step and the forehead point in subsequent ones. 
This strategy performs well in the initial two steps, with the performance in the first step nearing that of the one-step Oracle agent that adopts an ideal strategy.
TEPO-$3$ applies a nearly deterministic strategy that chooses the bounding box at the second step and chooses center points at other steps.
Moreover, TEPO-$5$ and TEPO-$7$ use more uncertain strategies that primarily employ the center point but may resort to alternative ones in the second and third steps.
TEPO-$9$ finds a trivial strategy of choosing the center point at each step, resulting in the best performance in multiple interactions.

\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.5\linewidth]{imgs/compare.png}
    \caption{Comparison of the number of cases with increased dice score less than $-0.1$.}
    \label{fig:misunderstand}
\end{figure}

\paragraph{Q\#d: How stable are the strategies learned by TEPO?}
One issue that may affect the performance of TEPO is interactive misunderstanding, where user interactions result in reduced segmentation dice scores.
In this study, we consider interactive misunderstandings when the segmentation dice score decreases by over $0.1$.
We analyze the occurrence of interactive misunderstandings for different strategies on our test data, as presented in Table \ref{tab:tepo_tab}.
For a more intuitive comparison, we plot the number of interactive misunderstandings for each strategy at different interaction steps in Figure \ref{fig:misunderstand}.
As TEPO-$2$ only applies to the initial two interactions, we exclude it from the plot.
Resultantly, the findings indicate that TEPO-$3$, TEPO-$5$, and TEPO-$7$ exhibit fewer misunderstandings than the random and alternating agents, thereby indicating superior stability and performance.

\subsubsection{Qualitative experimental analysis}
To evaluate the effectiveness of different strategies and investigate the causes of misunderstandings that occur with SAM, we conducted a qualitative analysis and present their performance on a single medical image in Figure~\ref{fig:case_study}.
The first column displays the raw image, while the middle columns show the interaction processes and corresponding segmentation outcomes. The last column provides the ground truth.
Among the different strategies, TEPO-$2$ demonstrates relatively weak performance, as it only involves two effective interactions.
The TEPO-$9$ and alternately changing agent purely used point-based interaction. TEPO-$9$ produces an equally good final outcome compared to the strategy with the bounding box and obtains the best result finally after nine interactions, the alternately changing policy performs poorly due to less effective interactions.
TEPO-$3$, and TEPO-$7$ consistently use the bounding box in the second interaction and select center points in all other interactions.
TEPO-$5$ uses the bounding box in the fourth interaction and center points in all other interactions. These three policies produce similar final results.
In addition, we observe a misunderstanding issue in some interactions, such as the seventh interaction with TEPO-$5$, and the eighth interaction with TEPO-$3$ and TEPO-$7$.
This is likely due to the corresponding region being too small for SAM to adequately understand the human feedback.

Overall, our results suggest that SAM cannot accurately achieve segmentation in a single interaction in medical tasks without being properly tuned. 
However, with multiple rounds of interaction, it can achieve considerable results. 
Moreover, the strategies learned by TEPO demonstrate better segmentation performance compared to rule-based strategies.
